CaBaFL: Asynchronous Federated Learning via Hierarchical Cache and Feature Balance

Federated Learning (FL) as a promising distributed machine learning paradigm has been widely adopted in Artificial Intelligence of Things (AIoT) applications. However, the efficiency and inference capability of FL is seriously limited due to the presence of stragglers and data imbalance across massive AIoT devices, respectively. To address the above challenges, we present a novel asynchronous FL approach named CaBaFL, which includes a hierarchical Cache-based aggregation mechanism and a feature Balance-guided device selection strategy. CaBaFL maintains multiple intermediate models simultaneously for local training. The hierarchical cache-based aggregation mechanism enables each intermediate model to be trained on multiple devices to align the training time and mitigate the straggler issue. In specific, each intermediate model is stored in a low-level cache for local training and when it is trained by sufficient local devices, it will be stored in a high-level cache for aggregation. To address the problem of imbalanced data, the feature balance-guided device selection strategy in CaBaFL adopts the activation distribution as a metric, which enables each intermediate model to be trained across devices with totally balanced data distributions before aggregation. Experimental results show that compared with the state-of-the-art FL methods, CaBaFL achieves up to 9.26X training acceleration and 19.71\% accuracy improvements.

==> comments.tex <==
\clearpage
\setcounter{section}{0}



\section{Responses to Reviewer Comments}
We would like to thank all the reviewers for their thoroughand insightful comments.
%We have revised the manuscript to address various issues raised by the reviewers. 
This section summarizes all the reviewer
comments and our responses in terms of how we have addressed the
issues in the revised manuscript. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.15 in}
\subsection{Reviewer 1}
\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment  1:} \textit{... explanation lacks clarity, particularly how exactly these patterns correlate with data distribution and the privacy implications thereof } 
% \textcolor{red}{TODO}
\end{tcolorbox}


\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
%We have modified the paper to make the explanation clearer (see page XXX). 
%
\textbf{Correlation between activation and data distributions:}
Typically, data of the same class have similar features, which in turn can activate the same neurons during the training. Based on this fact, our approach uses the activation distributions obtained from devices to indicate the data distributions on the devices. The observations in Section~\ref{sec:motivation} validate the such correlation between the activation and data distributions. 
%
\textbf{Explanation of privacy:} 
Although hard labels can reflect data distributions, we do not adopt them for device selection, since they can result in privacy leaks.
To achieve a wise device selection while avoiding the risk of privacy leakage, we adopt activation distributions for device selection.
This is mainly because i) according to observations in Section~\ref{sec:motivation}, activation distribution can be used to check the similarity of the data distribution between devices, and ii) it is extremely difficult for adversaries to restore the data distributions from the activation distributions since images of different classes can activate the same neurons and it is difficult to map the activation information to a specific data distribution without the raw data.
We have modified the paper and included the above explanations. 


% The DL model aims to extract the features of images and utilizes the extracted features for classification.
% Typically, images of the same class have similar features.
% In the inference process, when an image includes a specific feature, it can activate specific neurons.
% Therefore, images with the same class can activate similar neurons. Therefore, the distribution of activation can correlate with data distribution.
% The observations in our studies presented in Section~\ref{sec:motivation} demonstrate the above intuition.
% %
% \textbf{Explanation of the privacy:} 
% In this paper, CaBaFL aims to avoid exposing the distribution of client data. The activation information only counts the activation times of specific neurons for the local dataset, without including details of the input. Since images of different categories can activate the same neurons, activation information can be statistically related to the data distribution, but it cannot be used to restore it accurately.
% Furthermore, since the cloud server cannot access the local data, it is difficult to map the activation information to a specific data distribution. Therefore, compared to directly using data distribution, using activation information explores less privacy.



% Although activation has correlation with data distribution, the attackers cannot accurately restore the data distribution.
% % Compared to directly using data distribution, using activation can explore less privacy.
% This is mainly because images with different categories may activate the same part of neurons, so activation can be statistically related to the data distribution







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment  2:} \textit{... more information on privacy safeguards...} 
% \textcolor{red}{TODO}
\end{tcolorbox}


\vspace{-0.05 in}
\textbf{Response:} 
We agree that privacy is an important issue in FL design. Since this paper focuses on improving the overall learning performance, we did not consider additional privacy safeguards except activation distributions. Note that existing privacy safeguards can be easily integrated into our approach to protect its privacy.  




% From Section \ref{sec:motivation}, we know that even if the data has the same label distribution, its feature distribution may be very different. Therefore, uploading the feature distribution makes it difficult for the server to infer the label distribution of the local data on the device.


\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 3:} \textit{... system overhead, power consumption, and network usage ... in real AIoT environments.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Thanks for your suggestions. 
%
To further evaluate the performance of CaBaFL, we
conducted new experiments to measure more system metrics within a real 
 AIoT environment. Figures \ref{fig:real_devices_1.0} and \ref{fig:real_devices_iid} present the experimental results. We can find 
 that CaBaFL can still achieve the best performance compared to all the baselines (see page 10).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 4:} \textit{... considerable complexity in the proposed method... hinder reproducibility and practical application.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Since the two-level cache proposed in this paper is a logical concept, it does not introduce extra memory usage. Meanwhile, compared with the time complexity of  FL, the extra overhead caused by 
our device selection strategy is negligible. Therefore, the extra complexity will not hinder the reproducibility and practical application of our approach. 
To avoid confusion, we have included a more detailed time and memory complexity analysis of our approach in Section \ref{6.b}. 



% Our method does not have considerable complexity. Compared with the traditional FL algorithm, the additional time and memory complexity caused by our method is negligible. Therefore, our method is easy to reproduce and apply in practice. We added a more detailed time and memory complexity analysis to our paper, please see Section \ref{6.b} for more details (see page 11).




% We will analyze the complexity of our method from two aspects: time complexity and memory complexity. Assume that the dimension of feature distribution is $d$, the current round is the $k$-th round, the number of activated devices in a round is $n$, The number of all devices is $D$, and the number of parameters of the model is $m$.

% \textbf{Time complexity.} The time complexity of our method mainly comes from cache update and device selection. 1) Cache Update:  From Line 7 of Algorithm\ref{cabafl}, we can figure out that the time complexity of cache update is O($k\log k+d$). 2) Device Selection: From Lines 9-15 of Algorithm\ref{selectdevice}, we can determine the time complexity of device selection is O($n(d+n)$). Above all, the overall time complexity of our method is O($k\log k+d+n(d+n)$). Even for an FL system with 1000 devices, one round of cache update and device selection costs less than 2ms, which is negligible compared with local training time.

% \textbf{Memory complexity.} The memory complexity of our method mainly also comes from cache updates and device selection. i) Cache Update: Although there are two caches in our method, we can only maintain the L1 cache, and the L2 cache can only exist logically. Because the model in the L2 cache can be deleted from memory after being sent to the device for training. Therefore, the memory complexity is O($nm$). In addition, our method also maintains the model feature distribution and device feature distribution, and its memory complexity is O($(D+n)d$). 2) Device Selection: From Algorithm\ref{selectdevice}, we can determine that the memory complexity of device selection is O($Dd+n$). Since $nm\gg Dd+dn+n$, the overall memory complexity of our method is approximately O($nm$), which is the same as the one of traditional FL.

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 5:} \textit{... detailed discussion about the experimental setup, the selection of datasets, ... benchmarks used.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. To make a fair comparison with SOTA work, we adopt the experimental setup, datasets, and justification criteria in a similar manner. We have modified the paper and included more discussions on experimental settings (see page 6).



% i) The datasets we selected have wide applications and recognition in related work. Using these classic datasets enables us to effectively compare our method with baselines, enhancing the credibility and influence of our method. 
% ii) The benchmarks we selected include classic synchronous methods and the SOTA asynchronous and semi-asynchronous methods. The problems these baselines aim to solve are similar to those we aim to solve. Comparing these methods can effectively evaluate the effectiveness and advancement of our method.
% iii) We perform the same setup as [1]. And many papers use similar experimental setups [2]. We have added the above details in Section \ref{sec:5.a}(see page 6).

% {\color{blue}
% \footnotesize \noindent [1] M. Hu, et al. GitFL: Uncertainty-Aware Real-Time Asynchronous Federated Learning Using Version Control, RTSS, 2023.

% \footnotesize \noindent [2] K Luo, et al. GradMA: A gradient-memory-based accelerated federated learning with alleviated catastrophic forgetting, CVPR, 2023.
% }

\vspace{-0.1 in}
\subsection{Reviewer 2}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 1:} \textit{Uploading features to the center server imposes a huge communication burden ...}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} Sorry for the confusion.
In our approach, the devices upload the distribution of features instead of the features to the server. Specifically, after calculating the features of all images, the devices add up all the features to get the feature distribution and then upload this feature distribution to the server. Note that the size of the feature distribution is much smaller than the size of the feature.  
Therefore, the extra communication overhead is small and can be negligible. For example, assume that we use ResNet-18 for FL training. In this case, the dimension of a feature distribution is $(128\times2\times2)$. In other words, a device only needs to upload $128\times2\times2\times4=2048$B  data to the server.
We conducted new experiments to evaluate the communication overhead, and the results are shown in 
Figures \ref{fig:real_devices_1.0} and \ref{fig:real_devices_iid}. We can find that 
our method can achieve the best performance for a given communication overhead constraint. 



% Our method does not cause a huge communication burden. In our approach, the devices upload the distribution of features instead of the features to the server. Specifically, after calculating the features of all images, the devices add up all the features to get the feature distribution and then upload this feature distribution to the server. Note that the size of the feature distribution is much smaller than the size of the feature. For example, in our experiments using ResNet-18, the shape of the feature distribution is $(128\times2\times2)$. In other words, one device only needs to upload $128\times2\times2\times4$B of data to the server to update the feature distribution. Compared with the transmission model, the additional communication overhead caused by uploading feature distribution is negligible. 

% To demonstrate that our approach does not impose a huge communication burden, we measured the communication overhead of all devices using our real test bed. The result is shown in Figure \ref{fig:real_devices_1.0} and \ref{fig:real_devices_iid}. We can find that our method can achieve the best performance compared to all the
% baselines.



\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 2:} \textit{... wall clock time for training and other system-related metrics are not provided.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Thanks for your suggestion. The notion ``time'' in the figures indicates the wall clock time. 
We conducted new experiments to evaluate the energy consumption and communication overhead of all devices. The experimental results are shown in Figures~\ref{fig:real_devices_1.0} and \ref{fig:real_devices_iid}. We can find that our method can achieve the highest accuracy under the same energy consumption and communication overhead constraints.




\vspace{-0.1 in}
\subsection{Reviewer 3}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 1:} \textit{... lacks consideration for avoiding overfitting.}
\end{tcolorbox}
\vspace{-0.05 in}
%
\textbf{Response:} 
Indeed, overfitting is an important issue in FL training.
On the one hand, our method can easily integrate existing techniques to avoid overfitting, such as regularization.
On the other hand, our method considers the cosine similarity to the global feature distribution when updating the L2 cache, which can make the accumulated training data of the models involved in the aggregation more balanced. More balanced training data can effectively alleviate the gradient divergence problem caused by the non-IID problem so that the aggregated global model has better generalization, thereby alleviating the overfitting problem.
% We have modified the paper and included the above discussion (see page {\color{blue} XXX}). 



 
% Similar to most  FL methods,  our approach is based on FedAvg. Therefore, all the 
% existing methods to avoid overfitting can also be applied to our methods to address this issue.
% Furthermore,  when updating the L2 cache, our approach takes the cosine similarities between  
% local and global feature distributions into account. 
% In this way, the data accumulated across devices for training a model has a more balanced distribution,  thus effectively alleviating the gradient divergence problem caused by non-IID data on devices. Meanwhile, the overfitting problem is also alleviated. 




% the overfitting issue is a very common issue in FL. There are many common techniques, such as regularization and data augmentation, that can alleviate the overfitting problem. These techniques can be easily applied to our method.

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 2:} \textit{... workload imbalance among devices.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. Since our device selection strategy takes the fairness issue into account, our approach will not cause workload imbalance among devices.  
In our strategy, we use the hyperparameter $\sigma$ to control the activation of the device. During the FL training, if the variance of the number of device selections exceeds $\sigma$, CaBaFL will select idle devices that have been touched least frequently, ensuring the fairness of device selection. 
%
The results in  Figure \ref{fairness} show that our approach can treat devices in a fair manner. 
We have included the above explanation in Section \ref{sec:6.a} (see page 11).


% We recorded the number of times a device was selected using our device selection strategy
% and the random selection strategy, and the results are
% shown in Figure \ref{fairness}. 
%
% We can find that compared to the random selection strategy, except for a few outliers, the number of selected devices for our strategy is very close, demonstrating that the workload between devices is balanced. We have included the above explanation in Section \ref{sec:6.a} (see page 11).











\vspace{-0.1 in}
\subsection{Reviewer 4}

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 1:} \textit{Novelty is incremental in i) methods and ii) evaluation strategies.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. Our CaBaFL is a totally new solution 
to address two classic and important issues in FL, i.e., data imbalance among devices and the straggler problem.   

From the {\bf method} perspective, CaBaFL is based on a new asynchronous aggregation mechanism. 
Unlike traditional FL methods that aggregate models after their local training on one device. 
CaBaFL allows a model to be trained on multiple devices before an aggregation operation and uses a 
two-level cache to further improve the overall training performance. 
Moreover, CaBaFL proposes a new device selection strategy that uses feature distributions to 
  balance the training data accumulated across devices for models in a fine-grained way without privacy leakage. 
From the perspective of {\bf evaluation strategies}, to enable a fair and objective comparison with SOTA work, we adopt similar evaluation measurements as theirs. 
We have included the above discussion in the paper. 



% \textbf{Method.}
% CaBaFL is an innovative asynchronous federated learning method for the following reasons: 1) Our approach uses an innovative asynchronous aggregation mechanism. In traditional FL, the model is aggregated after being trained on one local device. However, in our approach, the model is aggregated after being trained on multiple devices. This can balance the training data and effectively alleviate the problem of data heterogeneity. In addition, we also designed a hierarchical cache to filter models to further effectively improve the global model accuracy. 
% 2) We have designed an innovative device selection mechanism based on feature balancing. Unlike traditional FL, our device selection mechanism balances data distribution by balancing feature distribution. Compared with the traditional FL algorithm that uses label distribution to balance data distribution, our algorithm can balance training data in a more fine-grained manner and does not require the server to obtain label distribution, which is private data.

% \textbf{Evaluation strategies.} We choose current evaluation methods based on their wide application and recognized effectiveness in related work. All baselines use similar evaluation strategies, which are widely regarded as being able to accurately and reliably evaluate the performance of related models and algorithms. Using these mature evaluation strategies ensures that our results are comparable and credible.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%









\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 2:} \textit{... experimental results using non-image datasets.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
%
Thank you for the suggestion. 
We conducted new experiments on a well-known dataset of table type named ``Activity'' using the MLP model. The experimental results are shown in Table \ref{tab:task_type}. We can find that 
CaBaFL still achieves the best accuracy (see page 9). 
% We have added this experiment to Section \ref{sec:5.c} .




% To further verify the effectiveness of our method on non-image datasets, we have applied our approach to the well-known table dataset Activity using the MLP model. Table \ref{tab:task_type} shows the experimental results. From this table, we can find that 






% \begin{table}[h]
% \vspace{-0.15 in}
% \centering
% \caption{Test accuracy on the Activity dataset.}
% \vspace{-0.1 in}
% \label{tab:activity}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|ccccccc|}
% \hline
% \multicolumn{7}{|c|}{Test Accuracy (\%)} \\ \hline
% \multicolumn{1}{|c|}{FedAvg} & \multicolumn{1}{c|}{FedProx} & \multicolumn{1}{c|}{FedASync} & \multicolumn{1}{c|}{FedSA} & \multicolumn{1}{c|}{SAFA} & \multicolumn{1}{c|}{WKAFL} & CaBaFL \\ \hline
% \multicolumn{1}{|c|}{$95.10\pm0.16$} & \multicolumn{1}{c|}{$95.23\pm0.12$} & \multicolumn{1}{c|}{$95.06\pm0.08$} & \multicolumn{1}{c|}{$95.27\pm0.09$} & \multicolumn{1}{c|}{$93.47\pm0.45$} & \multicolumn{1}{c|}{$95.17\pm0.76$} & $\textbf{95.43}\pm\textbf{0.23}$ \\ \hline
% \end{tabular}%
% }
% \vspace{-0.2 in}
% \end{table}



\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 3:} \textit{Quantification  ... stability and  fairness ...}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion.
We conducted new experiments to quantify the stability and fairness using the CIFAR-10 dataset and ResNet-18 model with $\beta = 0.5$. 

As shown in Table \ref{tab:stable}, we used the standard deviation of the Moving Average to quantify model stability for CaBaFL and all baselines. From this table, we can find the superiority of CaBaFL
in terms of stability. 
%
Meanwhile, our approach considers the fairness of device selection. 
% We use the variance of the number of times a device is selected to quantify model fairness. We calculated the performance of our device selection strategy and the random selection strategy on this metric. The metric of our device selection strategy is $8.7\times 10^{-7}$, and the metric of the random strategy is $10^{-6}$. $8.7\times 10^{-7}$ and $10^{-6}$ are very close, indicating that there is no fairness problem in our device selection strategy. We have included the above results in our paper (see page 7).
By introducing a hyperparameter $\sigma$, our device selection strategy can guarantee that each device can be selected with a similar number of times. We use the variance of the number of times a device is selected to quantify such fairness. the fairness of using our device selection strategy is $8.7\times 10^{-7}$, while the fairness of using the random strategy is $1\times10^{-6}$. This indicates the device selection strategy of  CaBaFL is fair.
We have included the above results in our paper (see page 7).







% i) Stability: We use the standard deviation of the Moving Average to quantify model stability. We calculated the performance of our method and all baselines on this metric, and the results are shown in Table \ref{tab:stable_re}.
 % ii) Fairness: We use the variance of the number of times a device is selected to quantify model fairness. We calculated the performance of our device selection strategy and the random selection strategy on this metric. The metric of our device selection strategy is $8.7\times 10^{-7}$, and the metric of the random strategy is $10^{-6}$. $8.7\times 10^{-7}$ and $10^{-6}$ are very close, indicating that there is no fairness problem in our device selection strategy. We have included the above results in our paper (see page 7).











\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 4\&5:} \textit{The Methodology section is hard to understand. Feature-guided device selection method for non-iid data is not clear.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. We have revised the methodology section and added more details about  
our feature-guided device selection methods (see pages 5 and 6). 


%When selecting devices, if the model $m_i$ has just started a new round of training, i.e., $c_i=0$, the server will randomly select a device for the model to start a new round of training. Otherwise, for each device $D_j$, CaBaFL calculates the cosine similarity $w_1$ when $D_j$ is selected between the feature distribution of model $m_i$ and the global feature distribution. Since the training time of a device is often proportional to its data size, balancing the model training data size can indirectly balance the training time between models in the L2 cache, thus mitigating the negative impact of stale models. Therefore, CaBaFL also considers balancing the training data size of models in the L2 cache when selecting devices. When selecting $D_j$, CaBaFL calculates the variance of the training data size of the models in the L2 cache, then subtracts $w_1$ from the variance to get the weight of the device, and selects the device with the highest weight for model scheduling. Finally, CaBaFL updates $S_{res}$, $f_{m_i}$ and $DS_i$. We have modified the paper to give a clearer explanation (see pages 5 and 6).

% \begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
% \textbf{Comment 5:} 
% \end{tcolorbox}

% \textbf{Response:} 

\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 6:} \textit{Several typos and grammatical errors ...}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} Thanks for pointing out the typos and grammar errors. We have scanned the paper carefully and corrected all of them. 


% modified Algorithm 1 and the relevant sentence to give a clearer statement (see pages 5 and 8).






\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 7:}\textit{ Figure 1, how (a) is different from (b) ... }
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
Figure~\ref{fig:motivation}(a) presents a training snapshot of some conventional synchronous FL methods, where local models are aggregated after they finish training on one activated device. In this case, the FL method performs two aggregation operations without taking the straggler problem into account. 
%
Unlike conventional FL methods, our approach considers the  straggler problem and 
allows a model to be trained on multiple devices before an aggregation operation. 
%
Meanwhile, when an activated device finishes its local training, it will immediately forward its hosting model to another device with balanced training overhead (see the implementation in Line 15 of Algorithm \ref{selectdevice}).
%
As an example shown in Figure~\ref{fig:motivation}(b), a model can traverse two devices before one aggregation operation, and all three models have similar overall training time on their two traversed devices. In this way, the straggler problem can be mitigated, since 
a compact training scheme can not only enable stragglers to be chosen for local training more often in a fair manner but also accelerate the training convergence processes. 
We have modified the paper and included the above explanation (see page 2). 









%%%%%%%%%%%%%%%


% In Figure 1(a), since the traditional synchronous aggregation process must wait for all activated devices to upload their local models, the training efficiency is limited by stragglers.
% To balance the training time, our motivation is to let a model be trained by multiple devices before aggregation and according to its training time for adaptive device selection.
% Specifically, if a model is trained by a straggler, it will be dispatched to a device with less training time for the next round of training and vice versa.
% Figure 1(b) illustrates our motivation, where the first model speeds the most training time in the first round and is dispatched to a device with less training time for the second round of training.
% After two rounds of training, all three models speed similar total time for local training.
% We have
% revised Figure \ref{fig:motivation} to demonstrate the difference in time cost between Figures \ref{fig:motivation}(a) and (b).





% Sorry for the confusion. Figure 1(a)
% shows a snapshot of some conventional synchronous FL scenarios, where
 
% %%%%%%%%%%%%
% {\color{red} In Figure 1, the red hollow arrow represents the model aggregation. We can see in Figure 1(a) that after the local model is trained on one local device, it is uploaded to the server for aggregation. However, in Figure 1(b), the local model is trained on multiple local devices before being uploaded to the server for aggregation. We have modified Section \ref{sec:3.a} to give a clearer statement (see page 2).
% }



\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 8:} \textit{... no clear architectural details where it shows how cache are organized. }
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
%
Inspired by the concept of cache in the computer architecture domain, we developed a novel two-level cache-like data structure that is hosted in the memory.  When a model is uploaded to the server, the server firstly stores it in the L2 cache. If the model 
has high quality as specified in Line 12 of Algorithm \ref{cabafl}, the server will move the model to the L1 cache.   
Note that in implementing CaBaFL, we do not create a large memory space for the two-level cache. Instead, the cache design is implemented based on the indices of local models. Since the local models are also required to be collected by traditional FL methods and the sizes of indices are much smaller than the models, the memory overhead of our cache design is negligible. 
We have modified Section \ref{sec:4.b} to include the above discussion (see page 5).



% In our approach, we maintain the L1 and L2 cache in the memory. When the model is uploaded to the server, the server first stores the model in the L2 cache. If the model meets certain conditions, the server updates the model to the L1 cache. Note that the L2 cache can just exist logically. Therefore, our method does not require additional space storage models compared to the traditional FL. 





\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 9:} \textit{... Where is novelty in terms of ... problem and solution? ... missed many recent works.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Indeed, our approach strives to solve two generic but important issues in FL, i.e., data imbalance and the straggler problem. However, our CaBaFL is a totally new solution 
to address two problems. 
Specifically,  CaBaFL is based on a new asynchronous aggregation mechanism. 
Unlike traditional FL methods that aggregate models after their local training on one device. 
CaBaFL allows a model to be trained on multiple devices before an aggregation operation and uses a 
two-level cache to further improve the overall training performance. 
Moreover, CaBaFL proposes a new device selection strategy that uses feature distributions to 
  balance the training data accumulated across devices for models in a more fine-grained way without privacy leakage. 
Compared with SOTA work, our approach can achieve better training performance.  

We agree that there are numerous works on similar problems. We have included and discussed more references (e.g., \cite{fedac,fedlc}) in the related work section to enrich the background of our approach. 





% %
% We illustrate the innovation of our approach from the perspectives of the straggler problem and the non-IID problem. i) straggler problem: Our method adopts an innovative asynchronous aggregation strategy to address the straggler problem.
% In a traditional asynchronous mechanism that aims to address the straggler problem, the local model is only trained on one device. However, in our approach, a model will be trained on multiple devices before being aggregated, which can reduce time lag and effectively address the straggler problem. ii) non-IID problem: 
% We have designed an innovative device selection mechanism based on feature balancing. Unlike traditional FL, our device selection mechanism balances data distribution by balancing feature distribution. Compared with the traditional FL algorithm that uses label distribution to balance data distribution, our algorithm can balance training data in a more fine-grained manner and does not require the server to obtain label distribution, which is private data.

% The paper you mentioned is an excellent and advanced method. Since it was not published when our paper was written, we did not add this paper to the related work. We have added this paper and more recent work to related work (see page 2).







\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 10:} \textit{... how authors address using the intermediate feature and computed similarity using cosine metric.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
According to the two observations in Section~\ref{sec:motivation}, 
the higher the  cosine similarity between the feature distribution of  training data 
and the global feature distribution, the more balanced 
the distribution of the accumulated training data is. 
%
Inspired by these findings, 
it is wise for the server to select devices that lead to high cosine similarities, which can effectively 
address the data imbalance problem. 
We have included the above discussion in Section \ref{sec:3.a}  (see page 4).


% From the motivation section, we know that the higher the cosine similarity between the feature distribution of the training data and the global feature distribution, the more balanced the training data is. Therefore, selecting a device that can make the cosine similarity between the feature distribution of training data and the global feature distribution high can make the training data distribution tend to be IID, thereby alleviating the non-IID problem. We have modified Section \ref{sec:3.a} to give a clearer statement (see page 4).


\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 11:}  \textit{Motivation is too long, but it's not clear why the proposal approach is necessary.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
%
Our approach strives to address two important issues in asynchronous FL, i.e., the straggler problem and
data imbalance problem. 
In the first part of our motivation, we illustrated a novel asynchronous FL mechanism that allows a model to be trained on multiple devices before an aggregation operation.
In this way, the straggler problem can be effectively mitigated. 
To further improve the training performance, 
the second part of our motivation tries to solve the data imbalance issue 
encountered during our proposed asynchronous aggregation. 
%
In this case, if the data accumulated across devices since the last aggregation operation to train each local model are evenly distributed, due to mitigation of ``weight divergence'' problems, 
the overall training performance will be significantly improved. 
Therefore, we investigated the correlation between the data distributions and activation distributions (i.e., feature distributions), aiming to optimize the device selection strategy so that the selected devices can achieve balanced accumulative training data for a given model. 
Note that due to the privacy issue, CaBaFL resorts to activation distributions rather than hard labels to reflect data distributions. We have modified the motivation section and included the above explanations.





% accumulated data  used to train local models are evenly distributed ,  


% aiming to make the
% total data used to train the model balanced before aggregation






% The reasons our approach is necessary are as follows: i) The asynchronous strategy of our approach can alleviate the straggler problem. In our approach, the model can be trained on multiple devices before aggregation, which can effectively reduce the time lag and alleviate the straggler problem. ii) Our approach can balance data distribution while preserving privacy. To alleviate the performance degradation caused by the non-IID problem, we need to balance the training data of the model. An intuitive way is to balance the distribution of training data by balancing the label distribution of the data. However, label distribution is often private information the server cannot obtain. Therefore, we innovatively balance the data distribution by balancing the feature distribution.








\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 12:}\textit{Methodology section should be improved, e.g., suddenly introduce the term ``cloud'', there is no explanation, Section IV.B first para is not required, but those details can be added to the algorithm itself, sims index how large and how often rewrite if required, no clarity}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. 
In the introduction section, we mentioned the ``cloud server'', which has the same meaning as the term ``server''.
%
In the revised version, we keep the first paragraph of Section IV.B, since we only have one paragraph to detail the algorithm for CaBaFL.  
%
Note that  $sims$ is a vector data structure maintained by the server. When receiving similarity information $sim_i$ from some device, the server will add $sim_i$ to  $sims$, and figure out the index of $sim_i$ within the sorted $sims$. 
We have modified the paper and included the above explanation in 
Section \ref{sec:4.b} (see page 5). 


% Every time we need to get the index of $sim_i$, we sort $sims$. Then we search $sim_i$ to get the index of $sim_i$. We have modified Section \ref{sec:4.b} to give a clearer statement .









\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comments 13\&14:} \textit{10\% devices... how is this valid for all stragglers? ... are all clients straggler or partially, no explanation.}
\end{tcolorbox}
\vspace{-0.05 in}
%
\textbf{Response:} 
Sorry for the confusion. In the experiments, we assume that 
10\% devices are randomly selected to perform simultaneous local training. 
%
To facilitate the evaluation, we assume that the training performance of all the devices follows a specific  Gaussian distribution. By default, 
our experiments assume that the training performance  (i.e., the training time of one data sample) of a device follows $N(0.03, 0.01)$, as measured in seconds. Note that in our approach, we did not explicitly specify the ratio of stragglers among all the devices, where a straggler only indicates a weak device with low training speed. In Figure \ref{fig:fig_extention},
we evaluate the impacts of different numbers of simultaneously training devices on the overall training performance. 
We have modified the paper and included the above explanations (see page 8). 


% \begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
% \textbf{Comment 14:} \textit{ }
% \end{tcolorbox}

% \textbf{Response:} Sorry for the confusion. In our experiments, some of the clients participating in training are stragglers.


\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 15:} \textit{Authors should add analysis on selected devices vs. accuracy vs. straggler percentage.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Thanks for your suggestion.  
{\bf Analysis of selected devices vs. accuracy:}
From Figure \ref{fig:fig_extention}, we can find that the stability of the accuracy of all the methods increases when more devices are selected. This is because the training data for the global model increases due to more selected devices, which alleviates the weight divergence problem. 
{\bf Analysis of straggler percentage vs. accuracy:}
From Table \ref{device}, we can find that the accuracy of baselines decreases when the number of dropouts increases. This is mainly because both synchronous and semi-asynchronous methods must wait for a certain number of models before aggregating. Therefore, their accuracy is affected by stragglers. Moreover, the number of stale models increased due to the increase in the number of stragglers, leading to a decrease in accuracy. We have included the above analysis in the paper (see page 8).






\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 16:}\textit{ Too many hyperparameters - how do you adjust them to achieve optimal performance? }
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} 
Sorry for the confusion. CaBaFL involves three hyperparameters (i.e., $\sigma$, $\gamma$, and $\alpha$), where increasing the values of the former two or decreasing the value of the last one can generally lead to better inference performance of the global model. Based on this fact,  we can randomly fix two parameters and tune the remaining one repetitively until reaching an expected performance.

 % When tuning parameters, we usually set an initial value based on experience, and then adjust each parameter in turn while fixing other parameters. When the current hyperparameter performs well, we fix this hyperparameter and adjust the next one.







\begin{tcolorbox}[notitle,boxrule=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=gray!20,colframe=gray!20]
\textbf{Comment 17:}  \textit{Section VI.B - complexity analysis is too vague as not considered actual computation.}
\end{tcolorbox}
\vspace{-0.05 in}
\textbf{Response:} Sorry for the confusion. 
We have improved the complexity analysis part and taken the actual computation into account. 
Please see Section \ref{6.b} for more details.


